Parameter Estimation via Conditional Expectation --- A Bayesian Inversion

When a mathematical or computational model is used to analyse some system, it is usual that some parameters resp.\ functions or fields in the model are not known, and hence uncertain. These parametric quantities are then identified by actual observations of the response of the real system. In a probabilistic setting, Bayes's theory is the proper mathematical background for this identification process. The possibility of being able to compute a conditional expectation turns out to be crucial for this purpose. We show how this theoretical background can be used in an actual numerical procedure, and shortly discuss various numerical approximations.

==> iformula.tex <==
%  hgm's macros

\newtheorem{thm}{Theorem}
%\newtheorem{thm}{Theorem}[section]
\newtheorem{xmpl}[thm]{Example}
\newtheorem{prop}[thm]{Proposition}
\newtheorem{rem}[thm]{Remark}
%\newtheorem{lemma}{Lemma}
\newtheorem{coro}[thm]{Corollary}
\newtheorem{schol}[thm]{Scholium}
\newtheorem{bei}[thm]{Beispiel}
\newtheorem{satz}[thm]{Satz}
\newtheorem{defi}[thm]{Definition}
\newtheorem{bem}[thm]{Bemerkung}
\newtheorem{lem}[thm]{Lemma}
\newtheorem{koro}[thm]{Korollar}

\newcommand{\ignore}[1]{}

\newcommand{\Wo}{\mathring{W}}
\newcommand{\Ho}{\mathring{H}}

\newcommand{\vrho}{\varrho}
\newcommand{\vepsilon}{\varepsilon}
\newcommand{\vsigma}{\varsigma}
\newcommand{\vtheta}{\vartheta}
\newcommand{\vphi}{\varphi}
\newcommand{\vpi}{\varpi}
\newcommand{\vkappa}{\varkappa}

%\newcommand{\vGamma}{\varGamma}
%\newcommand{\vDelta}{\varDelta}
%\newcommand{\vTheta}{\varTheta}
%\newcommand{\vLambda}{\varLambda}
%\newcommand{\vXi}{\varXi}
%\newcommand{\vPi}{\varPi}
%\newcommand{\vSigma}{\varSigma}
%\newcommand{\vUpsilon}{\varUpsilon}
%\newcommand{\vPhi}{\varPhi}
%\newcommand{\vPsi}{\varPsi}
%\newcommand{\vOmega}{\varOmega}

% math symbols

% slanted, bold, serifs (for vectors and matrices)
\newcommand{\vek}[1]{\mathchoice{\displaystyle\boldsymbol{#1}}
{\textstyle\boldsymbol{#1}}{\scriptstyle\boldsymbol{#1}}
{\scriptscriptstyle\boldsymbol{#1}}}

% upright, bold, serifs (usually not for variables), no lower case greek
\newcommand{\mat}[1]{\mathchoice{\displaystyle\mathbf{#1}}
{\textstyle\mathbf{#1}}{\scriptstyle\mathbf{#1}}
{\scriptscriptstyle\mathbf{#1}}}

% upright, bold, sans-serif (usually not for variables), no lower case greek
\newcommand{\opb}[1]{\vek{{\mathsf{#1}}}}

% upright, non-bold, sans-serif (usually not for variables), no lower case greek
\newcommand{\ops}[1]{\mathchoice{\displaystyle\mathsf{#1}}
{\textstyle\mathsf{#1}}{\scriptstyle\mathsf{#1}}
{\scriptscriptstyle\mathsf{#1}}}

% slanted, bold, sans-serif (for tensors)
\newcommand{\tnb}[1]{\mathchoice{\displaystyle\mathboldsans{#1}}
{\textstyle\mathboldsans{#1}}{\scriptstyle\mathboldsans{#1}}
{\scriptscriptstyle\mathboldsans{#1}}}

% slanted, non-bold, sans-serif (for tensor components)
\newcommand{\tns}[1]{\mathchoice{\displaystyle\mathsans{#1}}
{\textstyle\mathsans{#1}}{\scriptstyle\mathsans{#1}}
{\scriptscriptstyle\mathsans{#1}}}
 
\newcommand{\vcek}[1]{\vek{\check{#1}}}
\newcommand{\vbar}[1]{\vek{\bar{#1}}}
\newcommand{\vtil}[1]{\vek{\tilde{#1}}}
\newcommand{\vhat}[1]{\vek{\hat{#1}}}
 
\newcommand{\Mcek}[1]{\mat{\check{#1}}}
\newcommand{\Mbar}[1]{\mat{\bar{#1}}}
\newcommand{\Mtil}[1]{\mat{\tilde{#1}}}
\newcommand{\Mhat}[1]{\mat{\hat{#1}}}
 
\newcommand{\Tcek}[1]{\tnb{\check{#1}}}
\newcommand{\Tbar}[1]{\tnb{\bar{#1}}}
\newcommand{\Ttil}[1]{\tnb{\tilde{#1}}}
\newcommand{\That}[1]{\tnb{\hat{#1}}}
 
\newcommand{\Scek}[1]{\tns{\check{#1}}}
\newcommand{\Sbar}[1]{\tns{\bar{#1}}}
\newcommand{\Stil}[1]{\tns{\tilde{#1}}}
\newcommand{\Shat}[1]{\tns{\hat{#1}}}

\newcommand{\EXP}[1]{\mathbb{E}\left(#1\right)}
 
\newcommand{\dlangle}{\langle\negthinspace\langle}
\newcommand{\drangle}{\rangle\negthinspace\rangle}

\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}
\newcommand{\diag}{\mathop{\mathrm{diag}}\nolimits}
\newcommand{\grad}{\mathop{\mathrm{grad}}\nolimits}
\newcommand{\divg}{\mathop{\mathrm{div}}\nolimits}
\newcommand{\curl}{\mathop{\mathrm{curl}}\nolimits}
\newcommand{\rot}{\mathop{\mathrm{rot}}\nolimits}
\newcommand{\im}{\mathop{\mathrm{im}}\nolimits}
\newcommand{\dom}{\mathop{\mathrm{dom}}\nolimits}
\newcommand{\rank}{\mathop{\mathrm{rank}}\nolimits}
\newcommand{\tr}{\mathop{\mathrm{tr}}\nolimits}
\newcommand{\gra}{\mathop{\mathrm{gra}}\nolimits}
% \ker is already defined
% \dim is already defined
\newcommand{\coker}{\mathop{\mathrm{coker}}\nolimits}
\newcommand{\spn}{\mathop{\mathrm{span}}\nolimits}
\newcommand{\inti}{\mathop{\mathrm{int}}\nolimits}
\newcommand{\supp}{\mathop{\mathrm{supp}}\nolimits}
\newcommand{\sign}{\mathop{\mathrm{sign}}\nolimits}
\newcommand{\cl}{\mathop{\mathrm{cl}}\nolimits}
\newcommand{\acx}{\mathop{\mathrm{acx}}\nolimits}
\newcommand{\co}{\mathop{\mathrm{co}}\nolimits}

\newcommand{\dd}{\partial}
\newcommand{\di}{\mathrm{d}}
\newcommand{\Di}{\mathrm{D}}
\newcommand{\ii}{\mathchoice{\displaystyle\mathrm i}
{\textstyle\mathrm i}{\scriptstyle\mathrm i}
{\scriptscriptstyle\mathrm i}}
\newcommand{\ee}{\mathchoice{\displaystyle\mathrm e}
{\textstyle\mathrm e}{\scriptstyle\mathrm e}
{\scriptscriptstyle\mathrm e}}

